Curator Attack: When Blackbox Differential Privacy Auditing Loses Its Power

A surge in data-driven applications enhances everyday life but also raises serious concerns about private information leakage. Hence many privacy auditing tools are emerging for checking if the data sanitization performed meets the privacy standard of the data owner. Blackbox auditing for differential privacy is particularly gaining popularity for its effectiveness and applicability to a wide range of scenarios. Yet, we identified that blackbox auditing is essentially flawed with its setting: small probabilities or densities are ignored due to inaccurate observation. Our argument is based on a solid false positive analysis from a hypothesis testing perspective, which is missed out by prior blackbox auditing tools. This oversight greatly reduces the reliability of these tools, as it allows malicious or incapable data curators to pass the auditing with an overstated privacy guarantee, posing significant risks to data owners. We demonstrate the practical existence of such threats in classical differential privacy mechanisms against four representative blackbox auditors with experimental validations. Our findings aim to reveal the limitations of blackbox auditing tools, empower the data owner with the awareness of risks in using these tools, and encourage the development of more reliable differential privacy auditing methods.

==> 0_abstract.tex <==
\begin{abstract}
A surge in data-driven applications enhances everyday life but also raises serious concerns about private information leakage. Hence many privacy auditing tools are emerging for checking if the data sanitization performed meets the privacy standard of the data owner. Blackbox auditing for differential privacy is particularly gaining popularity for its effectiveness and applicability to a wide range of scenarios. Yet, we identified that blackbox auditing is essentially flawed with its setting --- small probabilities/densities are ignored due to inaccurate observation. Our argument is based on a solid false positive analysis from a hypothesis testing perspective, which is missed out by prior blackbox auditing tools. This oversight greatly reduces the reliability of these tools, as it allows malicious or incapable data curators to pass the auditing with an overstated privacy guarantee, posing significant risks to data owners. We demonstrate the practical existence of such threats in classical differential privacy mechanisms against four representative blackbox auditors with experimental validations. Our findings aim to reveal the limitations of blackbox auditing tools, empower the data owner with the awareness of risks in using these tools, and encourage the development of more reliable differential privacy auditing methods.
    \end{abstract}

==> 6_sniper_rappor.tex <==
\section{Example 3: One-time RAPPOR against DP-Sniper Auditing}
\label{sec:rappor_sniper}
\textbf{Benchmark RAPPOR Mechanism $M^{\text{rappor}}_{\theta}$.}
The benchmark claims to be $\epsilon_c$-DP and operates as in Alg. \ref{alg:rappor}. 
\begin{algorithm}[t]
    \SetAlgoLined
      \KwIn{Dataset $A$, parameter $\theta$, Bloom filter $B$ of size $k$, $h$ hash functions}
      \KwOut{$b$}
      Hash $A$ onto the Bloom filter $B$ using $h$ hash functions\;
      \For{each bit $B_i(A)$ in $B(A)$, $0\leq i < k$}{
        $b_i=1$ with probability $\frac{1}{2}\theta$; 
        $0$ with probability $\frac{1}{2}\theta$; $B_i(A)$ with probability $1-\theta$. 
      }
      Output $b$.
      \caption{One-time RAPPOR mechanism}
      \label{alg:rappor}
      \end{algorithm}

      \begin{theorem}
        \label{theorem:rappor_tight}
        The benchmark one-time RAPPOR mechanism $M^{\text{rappor}}_{\theta}$ is an FP against DP-Sniper auditing with probability threshold $c$ if 
        \begin{subequations}
          \begin{empheq}[left=\empheqlbrace]{align}
      & (P1)\ \ (\frac{1}{2}\theta)^{2h}< c, \label{eq:rappor_sniper_sub1}\\
      & (R1) \ \ 2h\cdot (\ln(1-\frac{1}{2}\theta)-\ln(\frac{1}{2}\theta)) > \epsilon_c,
       \label{eq:rappor_sniper_sub2}\\
      & (R2) \ \  
      (1-\frac{1}{2}\theta)^{2h}+q  h \theta (1-\frac{1}{2}\theta)^{2h-1}\leq e^{\epsilon_c }c.
      \label{eq:rappor_sniper_sub3}
          \end{empheq}
        \end{subequations}
    \end{theorem}
  \proof{
    ({P1}): We first determine the theoretical $S^*$ to solve for  prerequisite \ref{remark:1}. Intuitively, an output achieves the largest likelihood ratio when all $h$ bits in $B(a')$ differing from $B(a)$ are flipped. Formally, $\Pr[M^{\text{rappor}}_{\theta}(a')\in S^*]=(\frac{1}{2}\theta)^{2h}$, and {P1} becomes Eq. \eqref{eq:rappor_sniper_sub1}.

    ({R1}): The probability of dataset $a$ on the theoretical optimal outcome set $S^*$ is $\Pr[M^{\text{rappor}}_{\theta}(a)\in S^*]=(1-\tfrac{1}{2}\theta)^{2h}$.
     Hence the theoreotical DP level is $\epsilon^*(\theta)=\ln((1-\frac{1}{2}\theta)^{2h})-\ln((\frac{1}{2}\theta)^{2h})$, and R1 corresponds to Eq. \eqref{eq:rappor_sniper_sub2}.

    ({R2}): We now identify DP-Sniper's empirical $\hat{S}$. We denote the outcome set with the second largest ratio as $S'$, where $\Pr[M^{\text{rappor}}_{\theta}(a)\in S']=2h\cdot (1-\frac{1}{2}\theta)^{2h-1}\cdot(\frac{1}{2}\theta)$ and $\Pr[M^{\text{rappor}}_{\theta}(a')\in S']=2h\cdot (1-\frac{1}{2}\theta)\cdot(\frac{1}{2}\theta)^{2h-1}$. To simplify computation, we only consider $\theta$ for which $\Pr[M^{\text{rappor}}_{\theta}(a')\in S^*\cup S']\geq c$, in which case
    \begin{equation*}
          \Pr[b\in \hat{S}]=\mathbbm{1}[b\in S^*]+q\cdot\mathbbm{1}[b\in S'], \  q=\tfrac{c-\Pr[M^{\text{rappor}}_{\widetilde{\theta}}(a')\in S^*]}
          {
              \Pr[M^{\text{rappor}}_{\widetilde{\theta}}(a')\in S']  
          }.
      \label{eq:s_rappor}
   \end{equation*}
  Then $\xi^*(\widetilde{\theta})=\ln(\Pr[M^{\text{rappor}}_{\widetilde{\theta}}(a)\in S^*]+q\cdot \Pr[M^{\text{rappor}}_{\widetilde{\theta}}(a)\in S'])-\ln(c)$, and {R2} corresponds to Eq. \eqref{eq:rappor_sniper_sub3}.
  }

  
\textbf{Adapted RAPPOR Mechanism  (Omitted).} The only parameter involved in the one-time RAPPOR mechanism is the flipping probability $f$. Hence adapting a false positive mechanism reduces to identifying false positive benchmark RAPPOR, and we omit this redundant discussion.


